Optimal observables and estimators for practical superresolution imaging

Recent works identified resolution limits for the distance between incoherent point sources. However, it remains unclear how to choose suitable observables and estimators to reach these limits in practical situations. Here, we show how estimators saturating the Cram\'er-Rao bound for the distance between two thermal point sources can be constructed using an optimally designed observable in the presence of practical imperfections, such as misalignment, crosstalk and detector noise.

==> mode_picture.tex <==
\begin{tikzpicture}
\pgfmathdeclarefunction{gauss}{2}{%
  \pgfmathparse{1/(#2*(2*pi)^(1/4))*exp(-((x-#1)^2)/(2*#2^2))}%
}

\begin{axis}[
	at ={(0 cm, 2 cm)},
  	mark=none,
  	domain=-4:4,
  	samples=50,
  	smooth,
  	width=3 cm,
  	height=3 cm,
  	clip=false,
	%axis y line=none,
	%axis x line=none,
	ymax=1,
	ymin=-1,
	xtick=\empty,
	ytick=\empty,
	axis lines=middle,
	axis line style={->},
]
  \addplot [thick,red!70!black] ({x},{gauss(1,1)});
\end{axis}

\begin{axis}[
	at ={(0 cm, 0 cm)},
  	mark=none,
  	domain=-4:4,
  	samples=50,
  	smooth,
  	width=3 cm,
  	height=3 cm,
  	clip=false,
	%axis y line=none,
	%axis x line=none,
	ymax=1,
	ymin=-1,
	xtick=\empty,
	ytick=\empty,
	axis lines=middle,
	axis line style={->},
]
  \addplot [thick,red!70!black] ({x},{gauss(-1,1)});
\end{axis}

\begin{axis}[
	at ={(3 cm, 2 cm)},
  	mark=none,
  	domain=-4:4,
  	samples=50,
  	smooth,
  	width=3 cm,
  	height=3 cm,
  	clip=false,
	%axis y line=none,
	%axis x line=none,
	ymax=1,
	ymin=-1,
	xtick=\empty,
	ytick=\empty,
	axis lines=middle,
	axis line style={->},
]
  \addplot [thick,blue!70!black] ({x},{(gauss(-1,1)+gauss(1,1))/(sqrt(2)*(1 + 1/e^2))});
\end{axis}

\begin{axis}[
	at ={(3 cm, 0 cm)},
  	mark=none,
  	domain=-4:4,
  	samples=50,
  	smooth,
  	width=3 cm,
  	height=3 cm,
  	clip=false,
	%axis y line=none,
	%axis x line=none,
	ymax=1,
	ymin=-1,
	xtick=\empty,
	ytick=\empty,
	axis lines=middle,
	axis line style={->},
]
  \addplot [thick,blue!70!black] ({x},{(gauss(1,1)-gauss(-1,1))/(sqrt(2)*(1 - 1/e^2))});
\end{axis}

\begin{axis}[
	at ={(6 cm, 2 cm)},
  	mark=none,
  	domain=-4:4,
  	samples=50,
  	smooth,
  	width=3 cm,
  	height=3 cm,
  	clip=false,
	%axis y line=none,
	%axis x line=none,
	ymax=1,
	ymin=-1,
	xtick=\empty,
	ytick=\empty,
	axis lines=middle,
	axis line style={->},
]
  \addplot [thick,green!70!black] ({x},{gauss(0,1)});
\end{axis}

\begin{axis}[
	at ={(6 cm, 0 cm)},
  	mark=none,
  	domain=-4:4,
  	samples=50,
  	smooth,
  	width=3 cm,
  	height=3 cm,
  	clip=false,
	%axis y line=none,
	%axis x line=none,
	ymax=1,
	ymin=-1,
	xtick=\empty,
	ytick=\empty,
	axis lines=middle,
	axis line style={->},
]
  \addplot [thick,green!70!black] ({x},{2*x*gauss(0,1)});
\end{axis}

\node at (0.75, 1.75) {$u_0({\bf r} - {\bf r}_0)$};
\node at (0.75, 1.75-2) {$u_0({\bf r} + {\bf r}_0)$};
\node[red!70!black] at (0.75, 3.75) {Sources' images};

\node at (0.75+3, 1.75) {$w_0({\bf r}) = u_+({\bf r})$};
\node at (0.75+3, 1.75-2) {$w_1({\bf r}) = u_-({\bf r})$};
\node[blue!70!black] at (0.75+3, 3.75) {Auxiliary modes};

\node at (0.75+6, 1.75) {$v_0({\bf r}) = u_0({\bf r})$};
\node at (0.75+6, 1.75-2) {$v_1({\bf r}) = u_1({\bf r})$};
\node[green!70!black] at (0.75+6, 3.75) {Measurement modes};

\draw[thick, red!70!black] (-0.4, -0.5) rectangle (1.9, 3.5);
\draw[thick, blue!70!black] (-0.4+3, -0.5) rectangle (1.9+3, 3.5);
\draw[thick, green!70!black] (-0.4+6, -0.5) rectangle (1.9+6, 3.5);
\end{tikzpicture}

